To Trust or to Think: Cognitive Forcing Functions Can Reduce Overreliance on AI in AI-assisted Decision-making

People supported by AI-powered decision support tools frequently overrely on the AI: they accept an AI's suggestion even when that suggestion is wrong. Adding explanations to the AI decisions does not appear to reduce the overreliance and some studies suggest that it might even increase it. Informed by the dual-process theory of cognition, we posit that people rarely engage analytically with each individual AI recommendation and explanation, and instead develop general heuristics about whether and when to follow the AI suggestions. Building on prior research on medical decision-making, we designed three cognitive forcing interventions to compel people to engage more thoughtfully with the AI-generated explanations. We conducted an experiment (N=199), in which we compared our three cognitive forcing designs to two simple explainable AI approaches and to a no-AI baseline. The results demonstrate that cognitive forcing significantly reduced overreliance compared to the simple explainable AI approaches. However, there was a trade-off: people assigned the least favorable subjective ratings to the designs that reduced the overreliance the most. To audit our work for intervention-generated inequalities, we investigated whether our interventions benefited equally people with different levels of Need for Cognition (i.e., motivation to engage in effortful mental activities). Our results show that, on average, cognitive forcing interventions benefited participants higher in Need for Cognition more. Our research suggests that human cognitive motivation moderates the effectiveness of explainable AI solutions.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> discussion-revised.tex <==
\section{Discussion}

% Evaluate the assumptions that this work is based on
Consistent with prior research~\cite{bucinca20:proxy,green2019principles,lai2019human, bussone2015role}, our results demonstrate that people aided by simple explainable AI interfaces performed better overall than people who completed the task without any AI support. Also consistent with the prior research, these human+AI teams performed worse than the AI model alone (its accuracy was set to 75\%). Our results suggest that part of the reason is that people frequently overrelied on the AI: they followed the suggestions of the AI even when its predictions were incorrect. Consequently, when the AI predictions were incorrect, people aided by the simple explainable AI approaches performed less well than people who had no AI support. 

% Address the our claims (hypotheses)
% H1a: Compared to simple explainable AI approaches, cognitive forcing functions will improve the performance of human+AI teams in situations where the AI's top prediction is incorrect.
Our results demonstrate that cognitive forcing functions reduced over-reliance on AI compared to the simple explainable AI approaches: When the simulated AI model was incorrect, participants disregarded the AI suggestions and made the optimal choices significantly more frequently in the \emph{cognitive forcing function} conditions than in the \emph{simple explainable AI} conditions. These results \textbf{support the hypothesis (H1a).} 

However, even with the cognitive forcing functions, the human+AI teams in our study continued to perform worse than the AI model alone: the cognitive forcing functions reduced, but not yet eliminated, over-reliance on the AI.

% However, while cognitive forcing functions reduced over-reliance on the AI compared to the \emph{simple explainable AI} conditions, participants' performance when the model was incorrect was still significantly lower with \emph{cognitive forcing function} than that of participants in the \emph{no AI} condition. These findings suggest that cognitive forcing functions reduced, but not yet eliminated, over-reliance on the AI.

% H1b: Compared to simple explainable AI approaches, cognitive forcing functions will improve the performance of human+AI teams.

Our results \textbf{do not provide evidence to support the hypothesis (H1b)} that cognitive forcing functions will improve the performance of human+AI teams. There was no significant difference in performance between \emph{simple explainable AI} approaches and \emph{cognitive forcing functions}. %We speculate that the gain in performance on all questions was not significant, because the AI was mostly correct(~75 \%).  %Participants detected the carb source significantly better with \emph{cognitive forcing functions} compared to \emph{simple explainable AI} approaches and \emph{no AI} baseline. However, their overall performance, which in addition accounted for the whether an optimal ingredient was selected to replace the carb source with, was not significantly different from the simple explainable AI performance.
%We suspect that this might be partly due to the two decisions being different in nature: carb source detection was an \em objective \em decision as participants had to select the ingredient that was highest in carbs, whereas selecting the ingredient to replace it with involved assessing flavor similarity, which was a more \em subjective \em experience. Therefore, participants trusted and used the AI's suggestions in both categories more appropriately for the objective decisions, but not so for the \em subjective \em experience for which they did not perceive the AI to be as competent. This interpretation is in line with the recent work \cite{longoni2020artificial}, which demonstrated that people trust AI recommendations over human ones if they consider the utilitarian attributes of the choice, and human recommendations over AI ones if they consider the hedonic aspects of the choice.
%Because the AI mistakes stemmed form incorrect prediction of carb source, we think that the overall performance is less of an indicator of effectiveness of our interventions for reducing over-reliance compared to the carb source detection performance. 

%[[H1b is not supported, I think. We will need to address that. But I'd like to see the final graph of the overall performances of individual conditions first]]

% H2: There will be a negative correlation between the self-reported acceptability of the interface and the performance of human+AI teams in situations where the AI's top prediction is incorrect.
%Subjective ratings of the conditions indicate that participants in \emph{cognitive forcing function} conditions perceived the system as more complex than those in \emph{simple explainable AI} conditions. They also trusted the system in the \emph{simple explainable AI} conditions more. However, there was no significant difference between \emph{cognitive forcing functions} and \emph{simple explainable AI} conditions in terms of preference. 

Subjective ratings of the conditions indicate that participants in \emph{cognitive forcing function} conditions perceived the system as more complex than those in \emph{simple explainable AI} conditions.
The tension between subjective measures and performance is observed in the correlation analyses of  the subjective measures versus the performance. When the AI model was making incorrect predictions, people performed best in conditions that they preferred and trusted the least, and that they rated as the most difficult. Thus, \textbf{as hypothesized (H2)}, there appears to be a trade-off between the acceptability of a design of the human-AI collaboration interface and the performance of the human+AI team.

%NFC
 %They improved the performance of the less advantaged group -- people with lower NFC -- more than the performance of the group that was already predisposed to engage in analytical thinking. We assume that this might be due to the fact that people high in NFC were already more prone to engage analytically with the task and make better decisions even with no cognitive forcing. Hence, while cognitive forcing interventions improved their performance significantly for incorrect model predictions (i.e., reduced over-reliance), they did not have a significant effect on their performance on all questions.

%We assume that as the gain in performance from the extra effort was not substantial for people high in NFC, they preferred and trusted cognitive forcing interventions less than simple explainable AI approaches. Interestingly, this was not the case for people low in NFC. Their subjective ratings of trust and preference for cognitive forcing functions and simple explainable AI did not differ significantly. Yet, prior evidence suggests that people low in NFC do not prefer systems that present more information \cite{ghai2020explainable}. We speculate that cognitive forcing interventions might not have been perceived that way because by compelling people to reconsider their decisions, they made people realize their biases and that their initial decisions were suboptimal. Because these suboptimal decisions occurred more often for people with low NFC, they found cognitive forcing functions to be worth the extra cost of mental effort.


%%%%%%%% IMPLICATIONS, FUTURE WORK, LIMITATIONS %%%%%%%%%

% Immediate implications: importance of human factors in designing human+AI teams
Overall, our research suggests that human cognitive motivation moderates the effectiveness of explainable AI solutions. %More broadly, our results suggest that the effectiveness of human+AI collaborations on decision-making tasks depends on human factors that go beyond the choice of the right form and content of AI-generated explanations. 
Hence, in addition to tuning explanation attributes such as soundness and completeness~\cite{kulesza2013too}, or faithfulness, sensitivity, and complexity~\cite{bhatt2020evaluating}, explainable AI researchers should ensure that people will exert effort to attend to those explanations. 

%% Proxy tasks


Our results also lend further support to the recent research that demonstrated that using proxy tasks (where participants are asked, for example, to predict the output of an algorithm based on the explanations it generated) to evaluate explainable AI systems may lead to different results than testing the systems on actual decision-making tasks (where participants are asked to make decisions aided by an algorithm and its explanations)~\cite{bucinca20:proxy}. To explain their results, the authors hypothesized that proxy tasks artificially forced participants to exert effort and pay attention to the AI, but when participants were presented with actual decision-making tasks, they allocated fewer cognitive resources to analyzing AI-generated suggestions and explanations. %In our experiment, participants completed an actual decision-making task (i.e., they did not simulate the AI's decision) either with cognitive forcing interventions or without them and 
Our results showed that cognitive forcing interventions improved participants' ability to detect AI's errors in an actual decision-making task, where the human is assisted by the AI while making decisions. Hence, we concur: If we consider proxy tasks to be a strong form of a cognitive forcing intervention, our results suggest that evaluations that use proxy task are likely to produce more optimistic results (i.e., show higher human performance) than evaluations that use actual decision-making tasks with simple explainable AI approaches. 

%Ethical considerations
Because there is prior evidence that cognitively-demanding user interface interventions benefit people differently depending on the level of their cognitive motivation, we disaggregated our results by dividing our participants into two halves based on their Need for Cognition (NFC)---a stable personality trait that captures how much a person enjoys engaging in effortful cognitive activities. %Our research shows that inequalities among groups might be exacerbated by interventions in human-AI collaboration. 
The significant improvements in performance stemming from cognitive forcing functions we found, when disaggregated, held mostly for people with high NFC. %The effects of the interventions on performance was smaller for low-NFC group.  %Although, being external cognitive `motivators', we expected cognitive forcing functions to benefit more people with lower NFC, our results show that they benefit more people with a predisposition to engage in effortful cognitive activities. 
%Albeit, the people that benefited from cognitive forcing interventions the most, 
However, high-NFC participants trusted and preferred cognitive forcing functions less than simple explainable AI approaches, while there was no negative impact of these interventions on the low-NFC participants. These finding suggest that interventions might be tailored to account for the differences in intrinsic cognitive motivation: stricter interventions might benefit more and still be accepted by people with lower intrinsic cognitive motivation.

% Limitation: a non-critical tasks
A key limitation of our work is that it was conducted in the context of a single non-critical decision-making task. Additional work is needed to examine if the effects we observe generalize across domains and settings. However, because prior research provides ample evidence that even experts making critical decisions resort to heuristic thinking (and fall pray to cognitive biases)~\cite{berner2008overconfidence,bornstein2001rationality,croskerry2003importance,lambe2016dual}, we have some confidence that our results will generalize broadly.

% Future: adaptive
Another limitation is that cognitive forcing functions improved the performance of the human+AI teams at the cost of reducing the perceived usability. Consequently, systems that employ cognitive forcing functions may find less adoption than those that use simple explainable AI techniques because users will resist using them. We believe that this limitation could be overcome in part by developing \emph{adaptive} strategies where the most effective cognitive forcing functions are deployed only in a small fraction of cases where using them is predicted to substantially improve the final decision made by the human+AI team. Developing such adaptive strategies will require creating efficient models for predicting the performance of human+AI teams on particular task instances in the presence of different interventions. Our work suggests that these predictive models should consider AI's uncertainty for task instances and individual differences in cognitive motivation when predicting whether cognitive forcing functions are necessary.


